A new strategy for matching observed and simulated lensing galaxies

The study of strong-lensing systems conventionally involves constructing a mass distribution that can reproduce the observed multiply-imaging properties. Such mass reconstructions are generically non-unique. Here, we present an alternative strategy: instead of modelling the mass distribution, we search cosmological galaxy-formation simulations for plausible matches. In this paper we test the idea on seven well-studied lenses from the SLACS survey. For each of these, we first pre-select a few hundred galaxies from the EAGLE simulations, using the expected Einstein radius as an initial criterion. Then, for each of these pre-selected galaxies, we fit for the source light distribution, while using MCMC for the placement and orientation of the lensing galaxy, so as to reproduce the multiple images and arcs. The results indicate that the strategy is feasible, and even yields relative posterior probabilities of two different galaxy-formation scenarios, though these are not statistically significant yet. Extensions to other observables, such as kinematics and colours of the stellar population in the lensing galaxy, is straightforward in principle, though we have not attempted it yet. Scaling to arbitrarily large numbers of lenses also appears feasible. This will be especially relevant for upcoming wide-field surveys, through which the number of galaxy lenses will rise possibly a hundredfold, which will overwhelm conventional modelling methods.

==> fig/arrivs.tex <==
\begin{figure*}
    \addmosaic{arriv}{height=\qheight}
    \caption{Figure captions: Describe the graphics and tell why it's
    shown...}\figlbl{match:arriv}
  \end{figure*}

==> fig/data.tex <==
\begin{figure*}
    \addmosaic{data}{height=\pheight}
    \caption{Figure captions: Describe the graphics and tell why it's shown...}\figlbl{match:data}
\end{figure*}

==> fig/kappa.tex <==
% \begin{figure*}
%     \addmosaic{kappa}{height=\pheight}
%     \caption{Figure captions: Describe the graphics and tell why it's shown...}\figlbl{match:kappa}
% \end{figure*}

\begin{figure*}
    \centering
    \sidebysideA{kappa}{pixrad11}{height=\qheight}%
    \caption{Figure captions: Describe the graphics and tell why it's shown...}\figlbl{match:kappaA}
\end{figure*}

\begin{figure*}\ContinuedFloat
    \centering
    \sidebysideB{kappa}{pixrad11}{height=\qheight}%
    \caption{(Continued)}\figlbl{match:kappaB}
\end{figure*}

==> fig/pixrad11.tex <==
\begin{figure*}
    \addmosaic{pixrad11}{height=\pheight}
    \caption{Figure captions: Describe the graphics and tell why it's shown...}\figlbl{match:pixrad11}
\end{figure*}

==> fig/profiles.tex <==
\begin{figure*}
    \addmosaic{kprofile}{height=\qheight}
    \caption{Figure captions: Describe the graphics and tell why it's shown...}\figlbl{match:profiles}
\end{figure*}

==> fig/srcs.tex <==
% \begin{figure*}
%     \centering
%     \sidebysideA{srcplane}{resid}{height=\qheight}%
%     \caption{Figure captions: Describe the graphics and tell why it's shown...}\figlbl{match:srcsA}
% \end{figure*}

% \begin{figure*}\ContinuedFloat
%     \centering
%     \sidebysideB{srcplane}{resid}{height=\qheight}%
%     \caption{(Continued)}\figlbl{match:srcsB}
% \end{figure*}

\begin{figure*}
    \addmosaic{srcplane}{height=\qheight}
    \caption{Figure captions: Describe the graphics and tell why it's shown...}\figlbl{match:srcplane}
\end{figure*}

==> fig/synths.tex <==
% \begin{figure*}
%     \centering
%     \sidebysideA{data}{synth}{height=\qheight}%
%     \caption{Figure captions: Describe the graphics and tell why it's shown...}\figlbl{match:synthA}
% \end{figure*}

% \begin{figure*}\ContinuedFloat
%     \centering
%     \sidebysideB{data}{synth}{height=\qheight}%
%     \caption{(Continued)}\figlbl{match:synthB}
% \end{figure*}

\begin{figure*}
    \centering
    \triplecolA{data}{synth}{resid}{height=\qheight}%
    \caption{Figure captions: Describe the graphics and tell why it's shown...}\figlbl{match:synthA}
\end{figure*}

\begin{figure*}\ContinuedFloat
    \centering
    \triplecolB{data}{synth}{resid}{height=\qheight}%
    \caption{(Continued)}\figlbl{match:synthB}
\end{figure*}
